Finite-Time Analysis of Temporal Difference Learning with Experience Replay

Temporal-difference (TD) learning is widely regarded as one of the most popular algorithms in reinforcement learning (RL). Despite its widespread use, it has only been recently that researchers have begun to actively study its finite time behavior, including the finite time bound on mean squared error and sample complexity. On the empirical side, experience replay has been a key ingredient in the success of deep RL algorithms, but its theoretical effects on RL have yet to be fully understood. In this paper, we present a simple decomposition of the Markovian noise terms and provide finite-time error bounds for TD-learning with experience replay. Specifically, under the Markovian observation model, we demonstrate that for both the averaged iterate and final iterate cases, the error term induced by a constant step-size can be effectively controlled by the size of the replay buffer and the mini-batch sampled from the experience replay buffer.

==> app/tight_bound_avg_iterate.tex <==


\begin{theorem}[Convergence rate on average iterate of TD-learning]\label{thm:convergence_rate_average_TD_v2}
Suppose \(N>\max \{t^{\mathrm{mix}}_1,t^{\mathrm{mix}}_2\}\).
\begin{enumerate}
    \item[1)] For \(T \geq 0 \), the following inequality holds: 
    \begin{align}
      &\frac{1}{T}\sum_{k=0}^{T-1}    \mathbb{E}[||V_k-V^{\pi}||^2_2] \nonumber \\
     \leq & \frac{1}{T}\frac{2|\mathcal{S}|}{\alpha(1-\gamma)} \mathbb{E}[||V_0-V^{\pi}||^2_2] \nonumber \\
 & + \underbrace{\frac{32|\mathcal{S}|^{2}R_{\max}^2}{(1-\gamma)^3\mu^{\pi}_{\min}} 
\left(
 \sqrt{\frac{2\log(2|\mathcal{S}|)}{L}}+ \frac{2\log (2|\mathcal{S}|)}{3L}  
\right) }_{\text{$E^{\mathrm{avg}}_1$: Concentration error in the first moment}}+ \underbrace{\frac{32|\mathcal{S}|^{2}R_{\max}^2}{(1-\gamma)^3\mu^{\pi}_{\min}} \left(\sqrt{|\mathcal{S}|} \sqrt{\frac{t_1^{\mathrm{mix}}}{N}}
    +|\mathcal{S}|^{\frac{3}{2}}|\mathcal{A}|\sqrt{\frac{t^{\mathrm{mix}}_2}{N}} +\frac{64 t^{\mathrm{mix}}_1}{T}  \right) }_{ \text{$E^{\mathrm{avg}}_2$: Markovian noise in the first moment}}  \label{ineq_bias_term_avg_iterate_v2} \\
    &+ \underbrace{\alpha  \frac{4|\mathcal{S}|^2R^2_{\max}}{(1-\gamma)^3\mu^{\pi}_{\min}} \left(
 \frac{2|\mathcal{S}|}{L}+\frac{16|\mathcal{S}|}{9L^2}  
     \right)}_{\text{$E^{\mathrm{avg}}_3$: Concentration error in the second moment}}+  \underbrace{\alpha\frac{4|\mathcal{S}|^2R^2_{\max}}{(1-\gamma)^3\mu^{\pi}_{\min}}  \left(
|\mathcal{S}| \frac{t^{\mathrm{mix}}_1}{N} 
     +   2|\mathcal{S}|^4 |\mathcal{A}|^2\frac{t^{\mathrm{mix}}_2}{N} +
   \frac{32t_1^{\mathrm{mix}}}{T}  \right)}_{\text{$E^{\mathrm{avg}}_4$: Markovian noise in the second moment}}  \nonumber .
\end{align}
\item[2)]  For \(T \geq 0 \), the following inequality holds: 
  \begin{align}
  &   \mathbb{E} \left[ 
     \left\lVert 
     \frac{1}{T}
     \sum_{k=0}^T
     V_k-V^{\pi}
     \right\rVert_2
     \right] \nonumber
    \end{align}
\end{enumerate}
\end{theorem}

\begin{proof}

We prove the first item. Using~\eqref{eq:td_update_matrix}, we can expand \(  ||V_{k+1}-V^{\pi}||^2_M\) as follows:
\begin{align}
    ||V_{k+1}-V^{\pi}||^2_M &= (A(V_k-V^{\pi})+\alpha w(M_k^{\pi},V_k))^{\top} M (A(V_k-V^{\pi})+\alpha w(M_k^{\pi},V_k)) \nonumber \\
    &=(V_k-V^{\pi})^{\top} A^{\top}MA (V_k-V^{\pi}) + 2\alpha (V_k-V^{\pi})^{\top}A^{\top}Mw(M_k^{\pi},V_k) + \alpha^2 ||w(M_k^{\pi},V_k)||^2_M \nonumber \\
    &= ||V_k-V^{\pi}||^2_M -||V_k-V^{\pi}||^2_2
    + 2\alpha (V_k-V^{\pi})^{\top}A^{\top}M w(M_k^{\pi},V_k) + \alpha^2 ||w(M_k^{\pi},V_k)||^2_M \nonumber,
\end{align}
where the first equality follows from~\eqref{eq:td_update_matrix}, and the last equality follows from~\eqref{eq:A_discrete_lyap}. Taking expectation yields
\begin{align}
   &\mathbb{E}[||V_{k+1}-V^{\pi}||^2_M ] \nonumber \\
   =&\mathbb{E}[||V_k-V^{\pi}||^2_M] - \mathbb{E}[||V_k-V^{\pi}||_2]
   + 2\alpha \mathbb{E}[ (V_k-V^{\pi})^{\top}A^{\top}Mw(M_k^{\pi},V_k)]
   +\alpha^2 \mathbb{E}[|w(M_k^{\pi},V_k)||^2_M ] \nonumber\\
   \leq &\mathbb{E}[||V_k-V^{\pi}||^2_M] - \mathbb{E}[||V_k-V^{\pi}||_2]
   + 2\alpha \mathbb{E}[ (||MA
   (V_k-V^{\pi})||_2||w(M_k^{\pi},V_k)||_2 ]
   +\alpha^2 \mathbb{E}[|w(M_k^{\pi},V_k)||^2_M ] \nonumber\\
   \leq & \mathbb{E}[||V_k-V^{\pi}||^2_M] - \mathbb{E}[||V_k-V^{\pi}||_2]
   +  \alpha \frac{4\sqrt{|\mathcal{S}|}R_{\max}}{1-\gamma} ||MA||_2 \mathbb{E}[ ||w(M_k^{\pi},V_k)||_2 ]
   +\alpha^2 \mathbb{E}[|w(M_k^{\pi},V_k)||^2_M ] \nonumber\\
   \leq & \mathbb{E}[||V_k-V^{\pi}||^2_M ] - \mathbb{E}[||V_k-V^{\pi}||_2] +
      \frac{8|\mathcal{S}|^{\frac{3}{2}}R_{\max}}{(1-\gamma)^2\mu^{\pi}_{\min}}  \mathbb{E}[ ||w(M_k^{\pi},V_k)||_2 ]
   +\alpha
\frac{2|\mathcal{S}|}{(1-\gamma)\mu^{\pi}_{\min}}
   \mathbb{E}[|w(M_k^{\pi},V_k)||^2_2 ]  \nonumber\\
    \leq &   \mathbb{E}\left[ ||V_k-V^{\pi}||^2_M \right] -\mathbb{E}[||V_k-V^{\pi} ||^2_2] \nonumber \\
    &+ \frac{32|\mathcal{S}|^{2}R_{\max}^2}{(1-\gamma)^3\mu^{\pi}_{\min}} 
\left(
 2\sqrt{\frac{2\log(2|\mathcal{S}|)}{L}}  
    +2|\mathcal{S}|^{\frac{3}{2}}|\mathcal{A}|\sqrt{\frac{\max\{t^{\mathrm{mix}}_1,t^{\mathrm{mix}}_2\}}{N}} 
    +16|\mathcal{S}|d_{\mathrm{TV}}(\mu^{\pi}_{S_{\infty}},\mu^{\pi}_{S_{k-N}})
\right)   \nonumber \\
    &+  \alpha \frac{4|\mathcal{S}|^2R^2_{\max}}{(1-\gamma)^3\mu^{\pi}_{\min}}    \left(  \frac{4|\mathcal{S}|}{L} 
     +   4|\mathcal{S}|^4 |\mathcal{A}|^2\frac{\max\{t^{\mathrm{mix}}_1,t^{\mathrm{mix}}_2\}}{N}  
      +   8|\mathcal{S}| d_{\mathrm{TV}}(\mu^{\pi}_{S_{\infty}},\mu^{\pi}_{S_{k-N}})     \right) . \nonumber
\end{align}
where the first inequality follows from Cauchy-Schwartz inequality, and the second inequality follows from boundedness of \(V_k\) in~\Cref{lem:V_k_bdd}. The last inequality follows from bounding the first and second moment of \(\left\lVert w(M^{\pi}_k,V_k) \right\rVert_2\) by~\Cref{lem:first_moment_bound} and~\Cref{lem:second_moment_bound} respectively.

Using telescoping summation, we have
\begin{align}
 &\frac{1}{T^2}\sum_{k=0}^{T-1}    \mathbb{E}[||V_k-V^{\pi}||^2_2] \nonumber \\
 \leq &  \frac{1}{T^2}\mathbb{E}[||V_0-V^{\pi}||^2_M] \nonumber \\
 & + \frac{1}{T} \frac{32|\mathcal{S}|^{2}R_{\max}^2}{(1-\gamma)^3\mu^{\pi}_{\min}} 
\left(
2\sqrt{\frac{2\log(2|\mathcal{S}|)}{L}}+2|\mathcal{S}|^{\frac{3}{2}}|\mathcal{A}| \sqrt{\frac{\max\{t_1^{\mathrm{mix}},t^{\mathrm{mix}}_2\}}{N}}
\right) \nonumber\\
&+\frac{1}{T^2}\frac{32|\mathcal{S}|^{2}R_{\max}^2}{(1-\gamma)^3\mu^{\pi}_{\min}} 
\left( \sum_{k=0}^{T-1}16|\mathcal{S}| d_{\text{TV}}(\mu^{\pi}_{S_{\infty}},\mu^{\pi}_{S_{k-N}}) \right)
\nonumber\\
    &+ \frac{1}{T}\alpha  \frac{4|\mathcal{S}|^2R^2_{\max}}{(1-\gamma)^3\mu^{\pi}_{\min}} \left(
 \frac{4|\mathcal{S}|}{L}+ 2|\mathcal{S}|^4 |\mathcal{A}|^2 \frac{\max\{t^{\mathrm{mix}}_1,t^{\mathrm{mix}}_2\}}{N}   \right) \nonumber \\
    &+ \alpha \frac{1}{T^2} \frac{4|\mathcal{S}|^2R^2_{\max}}{(1-\gamma)^3\mu^{\pi}_{\min}} \left(
    \sum_{k=0}^{T-1}   16|\mathcal{S}| d_{\mathrm{TV}}(\mu^{\pi}_{S_{\infty}},\mu^{\pi}_{S_{k-N}}) \right) \nonumber.
\end{align}


To bound the sum of total variation terms, we use the following relation:
\begin{align}
     \sum_{k=0}^{T-1}d_{\mathrm{TV}}(\mu^{\pi}_{S_{\infty}},\mu^{\pi}_{S_{k-N}}) \leq t^{\mathrm{mix}}_1 \sum_{k=0}^{\lfloor T/t^{\mathrm{mix}}_1 \rfloor} d_{\mathrm{TV}}(\mu^{\pi}_{S_{\infty}},\mu^{\pi}_{S_{kt^{\mathrm{mix}}_1-N}})  
     \leq t^{\mathrm{mix}}_1 \sum^{\lfloor T/t^{\mathrm{mix}}_1 \rfloor}_{k=0} 2^{-k} \leq 2t^{\mathrm{mix}}_1. \label{ineq:sum_of_tv}
\end{align}

The first inequality follows from non-increasing property of total variation of irreducible and aperiodic Markov chain in~\Cref{lem:tv_mixing_time} in the Appendix. The second inequality follows from the first item in~\Cref{lem:tv_mixing_time} in the Appendix. 

\begin{align*}
     &\frac{1}{T^2}\sum_{k=0}^{T-1}    \mathbb{E}[||V_k-V^{\pi}||^2_2] \nonumber \\
     \leq & \frac{1}{T^2}\left(\frac{2|\mathcal{S}|}{\alpha(1-\gamma)} \mathbb{E}[||V_0-V^{\pi}||^2_2] +\frac{32^2|\mathcal{S}|^2R^2_{\max}}{(1-\gamma)^3\mu^{\pi}_{\min}} 4t^{\mathrm{mix}}_1 \right)\nonumber \\
 & + \frac{1}{T}\frac{32|\mathcal{S}|^{2}R_{\max}^2}{(1-\gamma)^3\mu^{\pi}_{\min}} 
\left(
2\sqrt{\frac{2\log(2|\mathcal{S}|)}{L}}  +2|\mathcal{S}|^{\frac{3}{2}}|\mathcal{A}| \sqrt{\frac{\max\{t_1^{\mathrm{mix}},t^{\mathrm{mix}}_2\}}{N}}
\right)   \nonumber\\
    &+ \frac{1}{T}\alpha  \frac{4|\mathcal{S}|^2R^2_{\max}}{(1-\gamma)^3\mu^{\pi}_{\min}} \left(
\frac{4|\mathcal{S}|}{L} + 2|\mathcal{S}|^4 |\mathcal{A}|^2 \frac{\max\{t^{\mathrm{mix}}_1,t^{\mathrm{mix}}_2\}}{N} \right)  \label{eq:avg_iterate_ss_1} .
\end{align*}

Now, note the following relation:
    
\begin{align}
  \mathbb{E} \left[ \left\lVert \frac{1}{T} \sum_{k=0}^{T-1} V_k-V^{\pi}\right\rVert^2_2 \right]
    \leq \frac{1}{T^2} \sum_{k=0}^{T-1}\mathbb{E}\left[\left\lVert V_k-V^{\pi}\right\rVert^2\right]
    + \frac{1}{T^2} \sum_{i=0}^{T-2}\sum_{j=i+1}^{T-1} \mathbb{E}\left[(V_i-V^{\pi})^{\top}(V_j-V^{\pi})\right]. \label{eq:avg_iterate_ss}
\end{align}

For \(0\leq i<j\leq T-1\) where \(\)Taking expectation, we need to bound \(    \mathbb{E}\left[  (V_i-V^{\pi})^{\top}(V_j-V^{\pi}) \right]\).

Note that
\begin{align*}
    V_j-V^{\pi} =& A(V_{j-1}-V^{\pi})+\alpha w(M_{j-1},V_{j-1})\\
                =& A^2 (V_{j-2}-V^{\pi})+\alpha Aw(M_{j-2},V_{j-2}-V^{\pi})+\alpha w(M_{j-1},V_{j-1})\\
                =& A^{j-i}(V_i-V^{\pi})
                +\alpha \sum_{k=1}^{j-i}  A^{k-1} w(M_{j-k},V_{j-k}) .
\end{align*}    

Now we can bound the crossing term, \((V_i-V^{\pi})^{\top}(V_j-V^{\pi})\) as follows:
\begin{align}
    &\mathbb{E}\left[ (V_i-V^{\pi})^{\top}(V_j-V^{\pi})  \right] \nonumber\\
=& \mathbb{E}\left[ (V_i-V^{\pi})^{\top}A^{j-i}(V_i-V^{\pi})+
\alpha (V_i-V^{\pi})^{\top}\left(\sum_{k=1}^{j-i}  A^{k-1} w(M_{j-k},V_{j-k})\right) \right]  \nonumber \\
    \leq &  \left\lVert A^{j-i} \right\rVert_2  
    \mathbb{E}\left[\left\lVert V_i-V^{\pi} \right\rVert^2_2  \right]
    +\alpha \mathbb{E}\left[ (V_i-V^{\pi})^{\top}\left(\sum_{k=1}^{j-i}  A^{k-1} w(M_{j-k},V_{j-k}) \right)\right]\\
    \leq & \sqrt{\mathcal{S}} (1-\alpha(1-\gamma)\mu^{\pi}_{\min})^{j-i}
    \mathbb{E}\left[\left\lVert V_i-V^{\pi} \right\rVert^2_2  \right] 
    +\alpha \frac{2R_{\max}\sqrt{S}}{1-\gamma} \mathbb{E}\left[
    \left\lVert \sum^{j-i}_{k=1} A^{k-1} w(M_{j-k},V_{j-k}) \right\rVert_2
    \right] \nonumber
    \\
    \leq & \sqrt{\mathcal{S}} (1-\alpha(1-\gamma)\mu^{\pi}_{\min})^{j-i}\mathbb{E}\left[\left\lVert V_i-V^{\pi} \right\rVert^2_2  \right] \nonumber \\
    &+ \alpha \frac{28|\mathcal{S}|^{\frac{3}{2}}R_{\max}^3}{(1-\gamma)^3} \sum^{j-i}_{k=1}  (1-\alpha(1-\gamma)\mu^{\pi}_{\min})^{k-1}   
     \left(  \frac{4|\mathcal{S}|}{|M^{\pi}_k
     |} +  4|\mathcal{S}|^4 |\mathcal{A}|^2\frac{\max\{t^{\mathrm{mix}}_1,t^{\mathrm{mix}}_2\}}{|B^{\pi}_k
     |} + 8|\mathcal{S}| d_{\mathrm{TV}}(\mu^{\pi}_{S_{\infty}},\mu^{\pi}_{S_{j-k-N}}) \right) \nonumber\\
\leq & \sqrt{\mathcal{S}} (1-\alpha(1-\gamma)\mu^{\pi}_{\min})^{j-i}\mathbb{E}\left[\left\lVert V_i-V^{\pi} \right\rVert^2_2  \right] \nonumber \\
&+ \frac{28|\mathcal{S}|^{\frac{3}{2}}R_{\max}^3}{(1-\gamma)^4\mu^{\pi}_{\min}}
\left( \frac{4|\mathcal{S}|}{|M^{\pi}_k
     |} 
     +   4|\mathcal{S}|^4 |\mathcal{A}|^2\frac{\max\{t^{\mathrm{mix}}_1,t^{\mathrm{mix}}_2\}}{|B^{\pi}_k
     |} \right)\\
     &+ \alpha \frac{224|\mathcal{S}|^{\frac{5}{2}}R_{\max}^3}{(1-\gamma)^3} (j-i) d_{\mathrm{TV}}(\mu^{\pi}_{S_{\infty}},\mu^{\pi}_{S_{i-N}})  \label{ineq:cross_term_bound}
\end{align}

Taking summation over the indices \(i\) and \(j\) results to
\begin{align}
    &\sum_{i=0}^{T-2}\sum_{j=i+1}^{T-1} \mathbb{E}\left[ (V_i-V^{\pi})^{\top}(V_j-V^{\pi}) \right] \nonumber\\
    =&\sum^{T-2}_{i=0} \sum_{j=i+1}^{T-1}
    \sqrt{\mathcal{S}} (1-\alpha(1-\gamma)\mu^{\pi}_{\min})^{j-i}\mathbb{E}\left[\left\lVert V_i-V^{\pi} \right\rVert^2_2  \right] \nonumber \\
&+ \frac{28|\mathcal{S}|^{\frac{3}{2}}R_{\max}^3}{(1-\gamma)^4\mu^{\pi}_{\min}}
\left( \frac{4|\mathcal{S}|}{L}+ 4|\mathcal{S}|^4 |\mathcal{A}|^2\frac{\max\{t^{\mathrm{mix}}_1,t^{\mathrm{mix}}_2\}}{N} \right) \nonumber\\
     &+ \alpha \frac{224|\mathcal{S}|^{\frac{5}{2}}R_{\max}^3}{(1-\gamma)^3} (j-i) d_{\mathrm{TV}}(\mu^{\pi}_{S_{\infty}},\mu^{\pi}_{S_{i-N}})\\
    \leq & \frac{\sqrt{\mathcal{S}}}{\alpha(1-\gamma)\mu^{\pi}_{\min}} \sum^{T-1}_{i=0} \mathbb{E}\left[ \left\lVert V_i-V^{\pi} \right\rVert^2_2\right]\nonumber\\ 
     &+T^2\frac{28|\mathcal{S}|^{\frac{3}{2}}R_{\max}^3}{(1-\gamma)^4\mu^{\pi}_{\min}}
\left( \frac{4|\mathcal{S}|}{L} + 4|\mathcal{S}|^4 |\mathcal{A}|^2\frac{\max\{t^{\mathrm{mix}}_1,t^{\mathrm{mix}}_2\}}{N}\right)\nonumber\\
     &+ T \alpha \frac{224|\mathcal{S}|^{\frac{5}{2}}R_{\max}^3}{(1-\gamma)^3} \sum^{T-1}_{i=0} d_{\mathrm{TV}}(\mu^{\pi}_{S_{\infty}},\mu^{\pi}_{S_{i-N}}) \nonumber\\
\leq & \frac{\sqrt{\mathcal{S}}}{\alpha(1-\gamma)\mu^{\pi}_{\min}} \sum^{T-1}_{i=0} \mathbb{E}\left[ \left\lVert V_i-V^{\pi} \right\rVert^2_2\right]\nonumber\\ 
     &+T^2\frac{28|\mathcal{S}|^{\frac{3}{2}}R_{\max}^3}{(1-\gamma)^4\mu^{\pi}_{\min}}
\left( \frac{4|\mathcal{S}|}{L} + 4|\mathcal{S}|^4 |\mathcal{A}|^2\frac{\max\{t^{\mathrm{mix}}_1,t^{\mathrm{mix}}_2\}}{N} \right)\\
     &+ T \alpha \frac{448t_1^{\mathrm{mix}}|\mathcal{S}|^{\frac{5}{2}}R_{\max}^3}{(1-\gamma)^3}  . \label{eq:avg_iterate_ss_2}
\end{align}

The first inequality results from~\eqref{ineq:cross_term_bound} and the second inequality follows from~\eqref{ineq:sum_of_tv}. 

Combining the results in~\eqref{eq:avg_iterate_ss_1} and~\eqref{eq:avg_iterate_ss_2}  to bound~\eqref{eq:avg_iterate_ss}, we get
\begin{align*}
&\mathbb{E} \left[ \left\lVert \frac{1}{T} \sum_{k=0}^{T-1} V_k-V^{\pi}\right\rVert^2_2 \right] \\
\leq & \frac{2\sqrt{\mathcal{S}}}{\alpha(1-\gamma)\mu^{\pi}_{\min}}
\left\{ \frac{1}{T^2}\left(\frac{2|\mathcal{S}|}{\alpha(1-\gamma)} \mathbb{E}[||V_0-V^{\pi}||^2_2]+\frac{32^2|\mathcal{S}|^2R^2_{\max}}{(1-\gamma)^3\mu^{\pi}_{\min}}4t^{\mathrm{mix}}_1\right)  \right.\\
&+ \frac{1}{T}\frac{32|\mathcal{S}|^{2}R_{\max}^2}{(1-\gamma)^3\mu^{\pi}_{\min}} 
\left(
2\sqrt{\frac{2\log(2|\mathcal{S}|)}{L}}  +|\mathcal{S}|^{\frac{3}{2}}|\mathcal{A}| \sqrt{\frac{\max\{t_1^{\mathrm{mix}},t^{\mathrm{mix}}_2\}}{N}}\right)  \\
&\left. + \frac{\alpha}{T}  \frac{4|\mathcal{S}|^2R^2_{\max}}{(1-\gamma)^3\mu^{\pi}_{\min}} \left(
\frac{4|\mathcal{S}|}{L} +   4|\mathcal{S}|^4 |\mathcal{A}|^2 \frac{\max\{t^{\mathrm{mix}}_1,t^{\mathrm{mix}}_2\}}{N} \right)\right\} \\
&+ \frac{28|\mathcal{S}|^{\frac{3}{2}}R_{\max}^3}{(1-\gamma)^4\mu^{\pi}_{\min}}
\left( \frac{4|\mathcal{S}|}{L} +  4|\mathcal{S}|^4 |\mathcal{A}|^2\frac{\max\{t^{\mathrm{mix}}_1,t^{\mathrm{mix}}_2\}}{N} \right)\\
&+\frac{\alpha}{T}\frac{448t_1^{\mathrm{mix}}|\mathcal{S}|^{\frac{5}{2}}R_{\max}^3}{(1-\gamma)^3}  .
\end{align*}


\begin{align*}
&\mathbb{E} \left[ \left\lVert \frac{1}{T} \sum_{k=0}^{T-1} V_k-V^{\pi}\right\rVert^2_2 \right] \\
\leq & \frac{2\sqrt{\mathcal{S}}}{\alpha(1-\gamma)\mu^{\pi}_{\min}}
\left\{ \frac{1}{T^2}\left(\frac{2|\mathcal{S}|}{\alpha(1-\gamma)} \mathbb{E}[||V_0-V^{\pi}||^2_2]+\frac{32^2|\mathcal{S}|^2R^2_{\max}}{(1-\gamma)^3\mu^{\pi}_{\min}}4t^{\mathrm{mix}}_1\right)  \right.\\
&+ \frac{1}{T}\frac{32|\mathcal{S}|^{2}R_{\max}^2}{(1-\gamma)^3\mu^{\pi}_{\min}} 
\left(
2\sqrt{\frac{2\log(2|\mathcal{S}|)}{L}}  +|\mathcal{S}|^{\frac{3}{2}}|\mathcal{A}| \sqrt{\frac{\max\{t_1^{\mathrm{mix}},t^{\mathrm{mix}}_2\}}{N}}\right)  \\
&\left. + \frac{\alpha}{T}  \frac{4|\mathcal{S}|^2R^2_{\max}}{(1-\gamma)^3\mu^{\pi}_{\min}} \left(
\frac{4|\mathcal{S}|}{L} +   4|\mathcal{S}|^4 |\mathcal{A}|^2 \frac{\max\{t^{\mathrm{mix}}_1,t^{\mathrm{mix}}_2\}}{N} \right)\right\} \\
&+ \frac{28|\mathcal{S}|^{\frac{3}{2}}R_{\max}^3}{(1-\gamma)^4\mu^{\pi}_{\min}}
\left( \frac{4|\mathcal{S}|}{L} +  4|\mathcal{S}|^4 |\mathcal{A}|^2\frac{\max\{t^{\mathrm{mix}}_1,t^{\mathrm{mix}}_2\}}{N} \right)\\
&+\frac{\alpha}{T}\frac{448t_1^{\mathrm{mix}}|\mathcal{S}|^{\frac{5}{2}}R_{\max}^3}{(1-\gamma)^3}  .
\end{align*}
\end{proof}


==> batch.tex <==

\begin{align}
    \mathbb{E}[||V^0_{k}-V^*||_2]
    \leq \mathbb{E}[||V^0_k - V^*_k||_2]
    + \mathbb{E}[||V^*_k - V^* ||_2] \nonumber
\end{align}
where \( V^*_k \) satisfies
\begin{align*}
    D_k V^*_k + \gamma D_kP_k V^*_k = D_k R
\end{align*}

\begin{align*}
    \mathbb{E}[ w_k^j\mid \mathcal{F}^j_{k-1},A]\mathbb{P}(A) + 
     \mathbb{E}[ w_k^j\mid \mathcal{F}^j_{k-1},A^c]\mathbb{P}(A^c)
\end{align*}

\begin{align}
    \mathbb{E}[w^j(M_k;V^j_k) \mid \mathcal{F}^j_{k-1}]
     = \frac{1}{N} \sum_{i=1}^N
     (e_s e_s)^{\top}( R + \gamma e_{s}P V_k - V_k) 
     -( D_k R + \gamma D_kP V_k - D_k V_k)
\end{align}
\begin{align*}
    \sum v_i f(O_i ;V_k)
\end{align*}
\begin{align*}
D_k R + \gamma D_k P^{\pi} V^*_k- D_k V^*_k
\end{align*}


==> coupling.tex <==

\begin{lemma}[i.i.d. bound of minibatch]
\begin{align*}
\mathbb{P}(\{w(\tilde{M}_k;\tilde{V}_k) \leq \epsilon \}|\tilde{\mathcal{F}}_{k-N})
\end{align*}
\end{lemma}
\begin{proof}
\begin{align*}
    \mathbb{E}\left[ \left\lVert  \frac{1}{L}\sum^L_{(s,a,s^{\prime})\in M_k} (e_{s,a}^{\top}(R+ e_{s^{\prime}}\gamma \Pi V_k - V_k)
-\tilde{D}_kR + \gamma \tilde{D}_k P\Pi_b V_k - \Tilde{D}_k V_k )\right\rVert_2  \middle| \mathcal{F}_{k-N}\right] \leq \epsilon
\end{align*}
\end{proof}

\begin{lemma}[Coupling of Markov chain]
Let \(O_1,O_2,\dots\) be a stationary Markov chain starting from stationary distribution \( \mu \). We can couple \((z_1,z_{K+1},z_{2k+1},\dots,z_{(n-1)K+1}) \) and \( (\tilde{z}_1,\tilde{z}_{K+1},\tilde{z}_{2K+1},\dots,\tilde{z}_{(n-1)K+1})   \).
\begin{align*}
    \mathbb{P}((z_1,z_{K+1},z_{2k+1},\dots,z_{(n-1)K+1}) \neq (\tilde{z}_1,\tilde{z}_{K+1},\tilde{z}_{2K+1},\dots,\tilde{z}_{(n-1)K+1}) ) \leq (n-1) d_{\mathrm{mix}}(K) 
\end{align*}
\end{lemma}

\begin{lemma}[Coupling buffer]
Coupling of buffer from Markov chain and i.i.d. buffer is:
\begin{align*}
    &\mathbb{P}(B_k \neq \tilde{B}_{k})\\
    &\iff \mathbb{P}((O_{k-N+1}.O_{k-N+2}.\dots,O_k))\neq (\tilde{O}_{k-N+1},\tilde{O}_{k-N+2}.\dots,\tilde{O}_k))
\end{align*}
Then
\begin{align*}
 &\mathbb{P}(\{O_i \neq \tilde{O}_i \}^k_{i=k-N+1}) \leq N d_{\mathrm{mix}}(L).
\end{align*}
\end{lemma}
\begin{proof}
\begin{align*}
    &\mathbb{P}(\{O_i \neq \tilde{O}_i \}^k_{i=k-N+1})\\
    &\leq \sum_{j=k-N+1}^{k-N+L} \mathbb{P}(\{  (O_{j+iL})_{i=0}^{N/L} \neq (\tilde{O}_{j+iL})_{i=1}^{N/L}   \} )
\end{align*}
\end{proof}
\begin{lemma}[Coupling Markov chain]
Consider a stationary Markov chain \( \{ O_1,O_2,\dots \} \), and we sampled \(M_k:=\{O_{1}^k,O_{2}^k,\dots,O_{L}^k\} \) from the replay buffer \( B_k:= \{O_{k-N},O_{k-N+1},\dots,O_{k} \} \). Then we can couple \( \tilde{B}_k:= \{\tilde{O}_{k-N},\tilde{O}_{k-N+1},\dots,\tilde{O}_{k}\} \sim \mu^{\otimes N}_{\infty}\) and sample
\( (\tilde{O}_{1}^k,\tilde{O}_{2}^k,\dots,\tilde{O}_{L}^k) \).
Suppose \( V_k = g (\mathcal{F}_{k-N},O_{k-N+1},\dots,O_{k-1} ) \), and 
\(\tilde{V}_k = g (\tilde{\mathcal{F}}_{k-N},\tilde{O}_{k-N+1},\dots,\tilde{O}_{k-1}) \), where
\begin{align*}
    \mathcal{F}_{k-N}&:=\{O_0,\dots,O_{k-N} \}\\
    \tilde{\mathcal{F}}_{k-N}&:=\{\tilde{O}_0,\dots,\tilde{O}_{k-N} \}
\end{align*}
\end{lemma}
\begin{proof}
Let \( M_k = (O_{1}^k,O_{2}^k,\dots,O_{L}^k )\) and 
\(\tilde{M}_k = (\tilde{O}_{1}^k,\tilde{O}_{2}^k,\dots,\tilde{O}_{L}^k)  \). Then,
\begin{align*}
&  \mathbb{P}( \{ ||w(M_k;V_k)|| \geq \epsilon \} \mid \mathcal{F}_{k-N} )\\
&=  \mathbb{P}( \{ ||w(M_k;V_k)|| \geq \epsilon \} \cap \{B_k=\tilde{B}_k \}  \mid \mathcal{F}_{k-N})\\
    &+\mathbb{P}( \{|| w(M_k;V_k)|| \geq \epsilon \} \cap \{B_k\neq \tilde{B}_k \} \mid \mathcal{F}_{k-N} )\\
    &\leq    \mathbb{P}(\{||w(\tilde{M}_k;V_k)|| \geq \epsilon \}\mid \mathcal{F}_{k-N})
    + \mathbb{P}(\{B_k\neq \tilde{B}_k \} \mid \mathcal{F}_{k-N})
\end{align*}

\end{proof}


\begin{lemma}
Consider a Markov chain \( O_1,O_2,\dots,O_k \) and replay buffer \(B_k = \{O_{k-N},O_{k-N+1},\dots,O_k\}\), and its mini-batch \( M_k:=\{O_{1}^k,O_{2}^k,\dots,O_{L}^k \}  \). Consider a stationary Markov chain \( \tilde{O}_1,\tilde{O}_2,\dots,\tilde{O}_k \) and replay buffer \(\tilde{B}_k = \{\tilde{O}_{k-N},\tilde{O}_{k-N+1},\dots,\tilde{O}_k\}\), and its mini-batch \( \tilde{M}_k:=\{\tilde{O}_{1}^k,\tilde{O}_{2}^k,\dots,\tilde{O}_{L}^k \}  \). 
\begin{align*}
    \mathcal{A} &: = \left\{ \mathbb{E}_{(x_i,u_i,x^{\prime}_i)}\left[ \left\lVert \frac{1}{L} \sum_{i=1}^L (  e_{x_i,u_i}^{\top}(R+ e_{x_i^{\prime}}\gamma \Pi V_k - V_k)
-\tilde{D}_{\infty}R + \gamma \tilde{D}_{\infty} P\Pi_b V_k - \Tilde{D}_{\infty} V_k 
    \right \rVert\right ] \geq \epsilon \right\} \\
        \mathcal{\tilde{A}} &: = \left\{ \mathbb{E}_{(\tilde{x}_i,\tilde{u}_i,\tilde{x}^{\prime}_i)}\left[\left\lVert \frac{1}{L} \sum_{i=1}^L (  e_{\tilde{x}_i,\tilde{u}_i}^{\top}(R+ e_{\tilde{x}_i^{\prime}}\gamma \Pi V_k - V_k)
-\tilde{D}_{\infty}R + \gamma \tilde{D}_{\infty} P\Pi_b V_k - \Tilde{D}_{\infty} V_k 
    \right \rVert\right]  \geq \epsilon \right\}
\end{align*}
\end{lemma}

\begin{proof}
Consider the following relation.
\begin{align*}
&\mathbb{P}(\{f(M_k;V_k)\leq \epsilon \}|O_{k-1}=o_{k-1},\dots,O_0=o_0,V_0=v_0)\\ &=\mathbb{P}(\{f(\tilde{M}_k;\tilde{V}_k) \leq \epsilon \})|\tilde{O}_{k-1}=o_{k-1},\dots,\tilde{O}_0=o_0,\tilde{V}_0=v_0) 
\end{align*}
Using the above relation we have
\begin{align*}
& \mathbb{P}_{k-2}(\{f(M_k;V_k)\leq \epsilon \})= \sum_{b} \mathbb{P}_{k-2}(\{f(M_k;V_k)\leq \epsilon \}|B_
{k-1} = b)\mathbb{P}_{k-2}(B_{k-1} = b)\\
&= \sum_{b} \mathbb{P}_{k-2}(\{f(\tilde{M}_k;\tilde{V}_k\geq \epsilon\})|\tilde{B}_
{k-1} = b)\mathbb{P}_{k-2}(B_{k-1} = b)\\
& \leq \sum_b \mathbb{P}_{k-2}(\{f(\tilde{M}_k;\tilde{V}_k) \geq \epsilon\}|\tilde{B}_{k-1}=b)\mathbb{P}(\tilde{B}_{k-1}=b) + \sum_b (\mathbb{P}_{k-2}(B_{k-1}=b) -\mathbb{P}(\tilde{B}_{k-1}=b))\\
&\leq \mathbb{P}_{k-2}(\{f(\tilde{M}_k;\tilde{V}_k) \geq \epsilon\})+\sum_z( \mathbb{P}_{k-2}(B_{k-1}=b) - \mu_{\infty} (b))
\end{align*}
We can bound if we do not start from stationary distribution.
\end{proof}


\begin{lemma}
Let
\begin{align*}
    \mathcal{A}:= \{||w(M_k;V_k)]|| \leq \epsilon \}.
\end{align*}
\end{lemma}

\begin{proof}
\begin{align*}
&    \mathbb{E}[w(M_k;V_k)\mid\mathcal{F}_{k-N}] \\   &=\mathbb{E}[w(M_k;V_k)\mid\mathcal{F}_{k-N},\mathcal{A}] \cdot \mathbb{P}_{k-N}(\mathcal{A})
+ \mathbb{E}[w(M_k;V_k)\mid\mathcal{F}_{k-N},\mathcal{A}^c] \cdot \mathbb{P}_{k-N}(\mathcal{A}^c)\\
&=\mathbb{E}[w(M_k;V_k)\mid\mathcal{F}_{k-N},\mathcal{A}] + W\delta
\end{align*}
\end{proof}

With replacement,
\begin{align}
    \mathbb{P}(\tilde{S}_i,\tilde{A}_i=(s,a)) = \frac{1}{L} \tilde{D}(s,a)
\end{align}

\begin{align}
    \mathbb{P}((s,a) \in RB_k) &= \frac{1}{N} \sum\limits^{N-1}_{i=0} 1\{(S_{k+i},A_{k+i})=(s,a)\} \nonumber\\
    &=\frac{1}{N} \sum\limits^{N-1}_{i=0}\mathbb{P}((S_{k+i},A_{k+i})=(s,a))=  \frac{1}{N} \sum_{i=k}^{i+N-1}d_i(s,a) \nonumber
\end{align}

\begin{align*}
    \mathbb{E}[e_{\tilde{S}_j,\tilde{A}_j}\mid B_k] &=  \sum_{(s,a)}\frac{1}{N}\sum\limits^{N-1}_{i=0} 1\{(S_{k+i},A_{k+i})=(s,a)\} e_{s,a}\\
    \mathbb{E}[e_{\tilde{S}_j,\tilde{A}_j}] & =\sum_{(s,a)}\frac{1}{N} \sum\limits^{N-1}_{i=0}\mathbb{P}((S_{k+i},A_{k+i})=(s,a))e_{s,a}= \sum_{(s,a)} \frac{1}{N} \sum_{i=k}^{i+N-1}d_i(s,a)e_{s,a}
\end{align*}

\begin{align}
    \mathbb{E}\left[
  \sum_{i=0}^{N-1} 1\{ (S_{k+i},A_{k+i} )= 
  (s,a)\} 
    \right] =   \sum_{i=k}^{i+N-1}d_i(s,a)
\end{align}


==> iid/iid.tex <==


Even though \(O_k\) is i.i.d., \(B_k\) are not i.i.d.. Instead, it forms a Markov chain:
\begin{align*}
    &\mathbb{P}(M_k,B_k\mid M_{k-1,}B_{k-1},M_{k-2},B_{k-2})\\
&=\mathbb{P}(M_k,X_{k},\dots,X_{k-N+1} \mid M_{k-1}, X_{k-1},\dots,X_{k-N-1},X_{k-N-2})\\
&=\mathbb{P}(M_k,X_{k},\dots,X_{k-N+1} \mid M_{k-1}, X_{k-1},\dots,X_{k-N-1})\\
&= \mathbb{P}(M_k,B_k \mid M_{k-1},B_{k-1})
\end{align*}


Note that \( \mathbb{P}(B_k\mid B_{k-1}) = \mathbb{P}(X_k) \).
Is \(\{B_k\}\) a uniform ergodic Markov chain? Yes since \( \mathbb{P}((M_k,B_k)=(m,b)\mid (M_{k-1},B_{k-1})=(m,b)) >0 \) for every possible \(m,b\).
\begin{lemma}
The Markov chain is irreducible and irreducible.
\end{lemma}
\begin{proof}
There exist \(k\) such that
\begin{align*}
&\mathbb{P}(M_{k}=m,B_{k}=b \mid M_0=m^{\prime},B_0=b^{\prime}) > 0.
\end{align*}

Aperiodicity can be checked for \(k\geq 0\).
\begin{align*}
    \mathbb{P}(M_{N+k}=m,B_{N+k}=b \mid M_0=m,B_0=b)>0.
\end{align*}

\end{proof}

\begin{algorithm}[H]
\caption{TD experience replay buffer i.i.d.}
\begin{algorithmic} 
\REQUIRE $B_{-1}:=O_{-N},O_{-N+1},\dots,O_{-1}$ data samples $V_0$;
\STATE $k=0$;
\FOR{$k\leq T$}
    \STATE Sample $B_k \sim \mathbb{P}(B_k \mid B_{k-1}) =\mathbb{P}(O_k)$
    \STATE Update \( V_k \)
\ENDFOR
\end{algorithmic}
\end{algorithm}

\begin{lemma}[Lipschitzness of Markovian noise term]
\begin{align*}
    ||w(M;V^{\prime})- w(M;V)||
\end{align*}
\end{lemma}
\begin{proof}
\begin{align*}
 &   \frac{1}{L}\left\lVert\sum^L_{(s,a,s^{\prime})\in M} ((e_{s}e_{s}^{\top})(R+\gamma  e_s e_{s^{\prime}}^{\top}V - V ) - D_{\infty}R + \gamma D_{\infty}P\Pi V - D_{\infty}V  ) \right.\\
&\left.
(e_{s}e_{s}^{\top})(R+\gamma  e_s e_{s^{\prime}}^{\top}V^{\prime} - V^{\prime} ) - D_{\infty}R + \gamma D_{\infty}P\Pi V^{\prime} - D_{\infty}V^{\prime} 
\right\rVert
\end{align*}
\end{proof}


\begin{lemma}[Lipschitzness of cross term]
\begin{align*}
   \xi(V,M) = (V-V^*)^{\top}w(M;V)
\end{align*}
is Lipschitz with respect to \(V\).
\end{lemma}

\begin{proof}
\begin{align*}
     &(V-V^*)^{\top}w(M;V)-  (V^{\prime}-V^*)^{\top}w(M;V^{\prime})\\
     &= (V-V^{\prime})^{\top} w(M;V)
     - (V^{\prime}-V^*)^{\top}(w(M;V^{\prime})-w(M;V))
\end{align*}
\end{proof}

Note that \(V_{k-N} \to B_{k-N} \to B_k \to M_k  \).


% Consider a coupling distribution \(B_k\) of \(\tilde{B}_k\). 



% \begin{align*}
%     &\mathbb{P}(M_k\mid M_{k-1}) =\sum_{B_k,B_{k-1}} \mathbb{P}(M_k,B_k,B_{k-1}\mid M_{k-1})\\
%     &= \sum_{B_k,B_{k-1}} \mathbb{P}(M_k\mid M_{k-1},B_k,B_{k-1})\mathbb{P}(B_k,B_{k-1}\mid M_{k-1})
% \end{align*}



% \begin{align*}
%      & \mathbb{E}[(V_k-V^*)^{\top}A^{\top}w_k\mid \mathcal{F}_{k-1} ]\\
%      &= (V_k-V^*)^{\top}A^{\top} \mathbb{E}[w_k\mid \mathcal{F}_{k-1}]\end{align*}


% Therefore we bound \(w_k\).
% \begin{align*}
% &\mathbb{E}[w_k \mid \mathcal{F}_0] =\mathbb{E}[\mathbb{E}[w_k\mid \mathcal{F}_1]\mid \mathcal{F}_0]
% \\ 
% &\mathbb{E}\left[  \frac{1}{L}\sum^L_{(s,a,s^{\prime})\in M_k} (e_{s,a}^{\top}(R+ e_{s^{\prime}}\gamma \Pi V_k - V_k)
% -\tilde{D}_{\infty}R + \gamma \tilde{D}_{\infty} P\Pi_b V_k - \Tilde{D}_{\infty} V_k ) \middle| \mathcal{F}_{k-1}\right] \\
% &= \mathbb{E}[f(M_k;V_k) \cdot 1\{ O_k\notin M_k\} \mid \mathcal{F}_{k-1}]+\mathbb{E}[f(M_k;V_k) \cdot 1\{ O_k \in M_k\} \mid \mathcal{F}_{k-1}]\\
% &= \mathbb{E}_{M_k\sim B_k\setminus O_k}[f(M_k;V_k)](1-1/N)^L+(1-(1-1/N)^L)\\
% &= \frac{N-1}{N}\frac{1}{L}\sum^L_{(s,a,s^{\prime})\in M_k} (e_{s,a}^{\top}(R+ e_{s^{\prime}}\gamma \Pi V_k - V_k)
% -\tilde{D}_{\infty}R + \gamma \tilde{D}_{\infty} P\Pi_b V_k - \Tilde{D}_{\infty} V_k )
% \end{align*}
% \(V_k\) is measurable w.r.t \(\mathcal{F}_{k-1}\).

% Now,
% \begin{align*}
%     &\mathbb{E}[f(M_k;V_k)\mid\mathcal{F}_{k-2}]\\
%     &= \mathbb{E}[\mathbb{E}[f(M_k;V_k)\mid\mathcal{F}_{k-1}]\mid\mathcal{F}_{k-2}]\\
%     &=\mathbb{E}\left[\frac{N-1}{N} f(M_k;V_k) \middle|\mathcal{F}_{k-2}\right]
% \end{align*}



==> iid/wo_replacemnt.tex <==


What we have to bound is 
\begin{align*}
    \left \lVert \mathbb{E} \left[\frac{1}{L}\sum_{i=1}^L (\delta (O^k_i;V_k) -\Delta(B_{\infty};V_k)) \middle | \mathcal{F}_{k-1}\right] \right \rVert.
\end{align*}

We decompose it into
\begin{align*}
     &   \left \lVert \mathbb{E} \left[\frac{1}{L}\sum_{i=1}^L (\delta (O^k_i;V_k) -\Delta(B_k;V_k)) \middle | \mathcal{F}_{k-1}\right] \right \rVert +  \left \lVert \mathbb{E}\left[
        \Delta(B_k;V_k) - \Delta (B_{\infty};V_k)
        \middle | \mathcal{F}_{k-1}\right] \right \rVert
\end{align*}

Later we will use the above to bound
\begin{align}
    \mathbb{E}\left[
     \left \lVert \mathbb{E} \left[\frac{1}{L}\sum_{i=1}^L (\delta (O^k_i;V_k) -\Delta(B_k;V_k)) \middle | \mathcal{F}_{k-1}\right] \right \rVert \middle| \mathcal{F}_{k-N}
    \right] \nonumber
\end{align}

\begin{lemma}
\begin{align*}
    &    \left \lVert \mathbb{E} \left[\frac{1}{L}\sum_{i=1}^L (\delta (O^k_i;V_k) -\Delta(B_k;V_k)) \middle | \mathcal{F}_{k-1}\right] \right \rVert \\
        & \leq
        \epsilon
\end{align*}
\end{lemma}
\begin{proof}
\begin{align*}
\end{align*}
\end{proof}


\begin{lemma}[Probability of event \(\{O_k\notin M_k \} \) under sampling without replacement]
\begin{align*}
    \mathbb{P}(O^k_i \neq O_k \mid \mathcal{F}_{k-1})
     = \frac{N-1}{N}
\end{align*}
\end{lemma}
\begin{proof}
Suppose we sample \( O^k_1 \) first. If \( O^k_1 = O_k \), then we are done. Otherwise , the process goes on.
\begin{align*}
\mathbb{P}(O^k_i\neq O_k \mid \mathcal{F}_{k-1})
 &= \frac{1}{N}+ \frac{N-1}{N}\frac{1}{N-1}
 + \dots \\
 &+
 \frac{N-1}{N}\frac{N-2}{N-1}\dots \frac{1}{N-i+1}
 +\frac{N-1}{N}\frac{N-2}{N-1}\dots \frac{N-i+1}{N-i}\frac{N-i}{N}\\
 &= \frac{N-1}{N}
\end{align*}
\end{proof}

\begin{lemma}[Expectation on TD error from \(N-1\) samples]
\begin{align*}
&\mathbb{E}[\delta (O^k_i;V_k) \mid \mathcal{F}_{k-1},O^k_i \neq O_k] \\
&= \frac{1}{N-1} (ND_{k-1}
-e_{s_{k-N}}e_{s_{k-N}}^{\top})
(R - V_k) +  \frac{1}{N-1}( ND_kP_k - e_{s_{k-N}}e_{s_{k-N}^{\prime}}^{\top} )\gamma  V_k
\end{align*}
\end{lemma}
\begin{proof}
\begin{align*}
    &\mathbb{E}[\delta (O^k_i;V_k) \mid \mathcal{F}_{k-1},O^k_i \neq O_k] \\
&=\left(\frac{1}{N-1} (ND_{k-1}
-e_{s_{k-N}}e_{s_{k-N}}^{\top})
(R - V_k) +    \frac{1}{N-1}( ND_kP_k - e_{s_{k-N}}e_{s_{k-N}^{\prime}}^{\top} )\gamma  V_k\right)\\
&= \frac{1}{N-1} (ND_{k-1}
-e_{s_{k-N}}e_{s_{k-N}}^{\top})
(R - V_k) +  \frac{1}{N-1}( ND_kP_k - e_{s_{k-N}}e_{s_{k-N}^{\prime}}^{\top} )\gamma  V_k
\end{align*}
Conditioning on \( \{ O^k_i \neq O_k \} \) implies that sampling \( O^k_i \) uniformly from \( B_{k-1} \setminus \{ (s_{k-N},s_{k-N}^{\prime} )\} \).
\end{proof}

\begin{lemma}[Expectation on mini-batch]
\begin{align*}
    &\mathbb{E} \left[\frac{1}{L}\sum_{i=1}^L (\delta (O^k_i;V_k) -\Delta(B_k;V_k)) \middle | \mathcal{F}_{k-1}\right]\\
    &=D_{k-1}+D_{k-1}P_{k-1}- D_{\infty}-D_{\infty}P
+ \frac{1}{N}((-e_{s_{k-N}}e_{s_{k-N}}^{\top})(R-V_k)- e_{s_{k-N}}e_{s_{k-N}^{\prime}}^{\top} \gamma  V_k) + \frac{1}{N}\Delta (V_k)
\end{align*}
\end{lemma}

\begin{proof}

\begin{align*}
    &\mathbb{E} \left[\frac{1}{L}\sum_{i=1}^L (\delta (O^k_i;V_k) -\Delta(B_k;V_k)) \middle | \mathcal{F}_{k-1}\right]\\
    &= \mathbb{E} \left[\frac{1}{L}\sum_{i=1}^L 1(O^k_i \neq   O_k)(\delta (O^k_i;V_k)-\Delta(B_k;V_k))\middle | \mathcal{F}_{k-1}\right] \\
    &=  \mathbb{E} \left[\frac{1}{L}\sum_{i=1}^L 1(O^k_i \neq   O_k)\delta (O^k_i;V_k) \middle | \mathcal{F}_{k-1}\right]
    -\mathbb{E}\left[\Delta(B_k;V_k) \frac{1}{L}\sum^L_{i=1}1(O^k_i\neq O_k)\middle | \mathcal{F}_{k-1}\right]\\
    &= \mathbb{E} \left[\frac{1}{L}\sum_{i=1}^L 1(O^k_i \neq   O_k)\delta (O^k_i;V_k) \middle | \mathcal{F}_{k-1}\right]
    - \Delta (V_k) \frac{1}{L}\sum_{i=1}^L \mathbb{P}(O^k_i\neq O_k \mid \mathcal{F}_{k-1})\\
    & = \mathbb{E} \left[\frac{1}{L}\sum_{i=1}^L 1(O^k_i \neq  O_k)\delta (O^k_i;V_k) \middle | \mathcal{F}_{k-1}\right]
    - \Delta (V_k)\frac{N-1}{N}\\
    &= \frac{1}{L}\sum_{i=1}^L \mathbb{E} \left[\delta (O^k_i;V_k) \middle | \mathcal{F}_{k-1},  O^k_i \neq o_k \right] \mathbb{P}(O^k_i \neq O_k \mid \mathcal{F}_{k-1})
    - \Delta (V_k)\frac{N-1}{N}\\
    &= \frac{1}{L} \sum^L_{i=1} \frac{N-1}{N} \left( \frac{1}{N-1} (ND_{k-1}
-e_{s_{k-N}}e_{s_{k-N}}^{\top})
(R - V_k) +  \frac{1}{N-1}( ND_{k-1}P_{k-1} - e_{s_{k-N}}e_{s_{k-N}^{\prime}}^{\top} )\gamma  V_k \right) \\
&- \Delta (V_k)\frac{N-1}{N}\\
&= \frac{1}{N}(ND_{k-1}
-e_{s_{k-N}}e_{s_{k-N}}^{\top})(R-V_k) + \frac{1}{N}(ND_{k-1}P_{k-1} - e_{s_{k-N}}e_{s_{k-N}^{\prime}}^{\top} )\gamma  V_k - \frac{N-1}{N}\Delta (V_k)\\
&= D_{k-1}+D_{k-1}P_{k-1}- D_{\infty}-D_{\infty}P
+ \frac{1}{N}((-e_{s_{k-N}}e_{s_{k-N}}^{\top})(R-V_k)- e_{s_{k-N}}e_{s_{k-N}^{\prime}}^{\top} \gamma  V_k) + \frac{1}{N}\Delta (V_k)
\end{align*}

The first inequality follows since when \( O^k_i= O_k \), then
\begin{align*}
&    \mathbb{E}[\delta(O^k_i;V_k) - \Delta (B_k;V_k) \mid \mathcal{F}_{k-1},\{O^k_i=O_k \}]\\
&= -(D_k+D_{\infty})(R-V_k) - (D_kP_k - D_{\infty}P)V_k
\end{align*}

\end{proof}


\begin{lemma}
\begin{align*}
\mathbb{E}[||\mathbb{E}[w(M_k;V_k) \mid\mathcal{F}_{k-1}] \mid \mathcal{F}_{k-N} ] ||\leq
\end{align*}
\end{lemma}
\begin{proof}
\begin{align*}
    \mathbb{E}[|| D_{k-1} - D_{\infty} + D_{k-1}P_{k-1} - D_{\infty}P ||\mid \mathcal{F}_{k-N}] \leq \epsilon_1 + \epsilon_2 + 2( 1-\delta_1 ) + 2 (1-\delta_2 ) 
\end{align*}
\end{proof}


Therefore,

\begin{align*}
   \frac{1}{N-1}( ND_kP_k - e_{s_{k-N}}e_{s_{k-N}^{\prime}}^{\top} )
\end{align*}



\begin{lemma}
\begin{align*}
    &\mathbb{E}[|| D_{k-1}-D_{\infty}||_{\infty}+ || D_{k-1}P_{k-1}- D_{\infty}P ||_{\infty} \mid \mathcal{F}_{k-N-1}] \\
    &\leq
    \epsilon_1 + \epsilon_2 + 2 (1-\delta_1) + 2(1-\delta_2)
\end{align*}
\end{lemma}

\begin{proof}
Using maximal Azuma Hoeffding inequality,
\begin{align*}
    &\mathbb{P}( || D_{k-1}-D_{\infty}||_{\infty} \geq \epsilon_1 ) 
    \leq \sum_s \mathbb{P}(|\mu_k(s)-\mu(s)| \geq \epsilon_1 )\\
 &= \sum_s \mathbb{P}\left(\left| \frac{\sum_i 1(s_i=s)}{N}-\mu(s) \right|   \geq\epsilon_1 \right)\\
 &=2 |\mathcal{S}|  \exp( -\epsilon^2/(2N) ) 
\end{align*}

Therefore, 
\begin{align*}
&    \mathbb{E}[||D_{k-1}-D||_{\infty}\mid \mathcal{F}_{k-N-1}]
    =\mathbb{E}[||D_{k-1}-D||_{\infty}]\\
&= \mathbb{E}[||D_{k-1}-D||_{\infty}\mid \mathcal{A}]\mathbb{P}(\mathcal{A})
+\mathbb{E}[||D_{k-1}-D||_{\infty}\mid \mathcal{A}^c]\mathbb{P}(\mathcal{A}^c)\\
&\leq \epsilon_1 + 2 ( 1-\delta_1 )
\end{align*}
\end{proof}

As a result we get
\begin{align}
&    \mathbb{E}[||V_{k+1}-V^*||^2_2] \leq (1-\alpha_k \rho ) \mathbb{E}[|| V_k - V^*||^2] + \epsilon \alpha_k + \alpha_k^2 W\\
&  \rho \alpha_k \mathbb{E}[||V_k-V^*||^2] \leq  \mathbb{E}[||V_k-V^*||^2] -  \mathbb{E}[||V_{k+1}-V^*||^2] + \epsilon \alpha_k + \alpha_k^2 W\\
& \rho \sum  \alpha_k \mathbb{E}[||V_k-V^*||^2]  \leq \mathbb{E}[||V_0-V^*||^2]
+ \epsilon \sum_k \alpha_k + \sum_k \alpha_k^2 W
\end{align}


==> markovian.tex <==

\subsection{Markov process}
\begin{lemma}[Ergodicity of replay buffer~\citep{di2022analysis}]
\( \{B_1,B_2,\dots,\}\) is time homoeneous irreducible and aperiodic Markov chain. i.e., it mixes uniformly.
\end{lemma}

\begin{proof}

\begin{align*}
    \mathbb{P}(B_{k+1}\mid B_k) 
    \begin{cases}
    0 &  \text{if not realizable}\\
    \mathbb{P}(X_{k+1} \mid X_k) & \text{if realizable}
    \end{cases}
\end{align*}

Irreducibility can be seen easily from the fact that \(X\) is irreducible. Aperiodicity can be alos chekced since \(X\) is aperiodic.. 
\end{proof}

\begin{lemma}
Let \(M^{\prime}_k\) and \(V^{\prime}_{k-N}\) be independent copies drawn from marginal distributions of \(M_k\) and \( V_{k-N}\).
\begin{align*}
\mathbb{E}[\xi(M_k;V_{k-N})] \leq 2\Xi m\rho^N
\end{align*}
\end{lemma}

\begin{proof}
From the control of coupling lemma, we have
\begin{align*}
   |  \mathbb{E}[\xi(M_k;V_k)] - \mathbb{E}[\xi(M_k^{\prime};V_{k-N}^{\prime})]   | \leq 2\Xi m\rho^N
\end{align*}
Here we use the fact that
\begin{align}
    \mathbb{E}[\xi(M_k^{\prime};V_{k-N}^{\prime})]= \mathbb{E}[ \mathbb{E}[\xi(M_k^{\prime},V^{\prime}_{k-N})\mid V^{\prime}_{k-N} ]] =0  \nonumber.
\end{align}
\end{proof}

\begin{lemma}
\begin{align*}
    \mathbb{E}[\xi(M_k;V_k)] \leq m\rho^{N} +\Xi_L NG \alpha_{k-N}
\end{align*}
If \( N = \mathcal{O}(\log k )\), then 
\begin{align*}
    \mathbb{E}[\xi(M_k;V_k)] \leq \mathcal{O}\left( \frac{\log k}{k} \right)
\end{align*}
\end{lemma}

\begin{proof}
\begin{align*}
    &V_i - V_{i-1} = \alpha_i (-DV_{i-1} + DPV_{i-1} + w(M_{i-1};V_{i-1})) \to ||V_i-V_{i-1}||_2 \leq \alpha_i G\\
    &||V_k - V_{k-N}||_2 \leq \sum_{i=k-N}^{k-1} \alpha_i G \leq NG \alpha_{k-N} \\
    & \xi(M_k;V_k) \leq \xi(M_k;V_{k-N}) + \Xi_L || V_k - V_{k-N}||_2
\end{align*}
Taking expectation,
\begin{align*}
    \mathbb{E}[\xi(M_k;V_k)] \leq \mathbb{E}[\xi(M_k;V_{k-N})] + \Xi_L NG \alpha_{k-N} \leq m\rho^{N} +\Xi_L NG \alpha_{k-N}
\end{align*}

\end{proof}


==> misc.tex <==
\subsection{Mini-batch as Markov chain}


\begin{definition}[\(f\)-divergence] \(f :0 \to [0,\infty]\) and convex function and \(f(1)=0\). The \(f\)-divergence is defined as
\begin{align*}
    d_f (P||Q) = \int f\left(\frac{dP}{dQ}\right)dQ.
\end{align*}
\end{definition}

\begin{remark}
If \( f(x) = |x-1|/2 \), then it becomes total-variation distance.
\end{remark}


\begin{lemma}[Data-processing inequality]
If \( X \to Y\to Z \),
\begin{align*}
    I_f (X,Z) \leq I_f(X,Y).
\end{align*}
\end{lemma}


\begin{lemma}[Control of coupling]
Consider a 
\begin{align*}
    X \to B_k \to B_{k+\tau} \to Y
\end{align*}
Then,
\begin{align*}
    | \mathbb{E}[v(X,Y)]- \mathbb{E}[v(X^{\prime},Y^{\prime})] \leq 2 ||v||_{\infty} (m\rho^{\tau}).
\end{align*}
\end{lemma}


\begin{remark}[Backward Markov chain]
\begin{align*}
    \mathbb{P}(Z_{k-1}|Z_k,Z_{k+1}) &= \mathbb{P}(Z_{k+1},Z_k,Z_{k-1})/\mathbb{P}(Z_k,Z_{k+1})\\
    &=\mathbb{P}(Z_{k+1}|Z_k,Z_{k-1})\mathbb{P}(Z
    _k,Z_{k-1})/\mathbb{P}(Z_k,Z_{k+1})\\
    &=\mathbb{P}(Z_k,Z_{k-1})/\mathbb{P}(Z_k)=\mathbb{P}(Z_{k-1}|Z_k)\\
    &= \mathbb{P}(Z_k|Z_{k-1})\mathbb{P}(Z_{k-1})/\mathbb{P}(Z_k)
\end{align*}
\end{remark}

\begin{lemma}\label{lem:concentration_iid}[Concentration bound for i.i.d. vectors]
Let \( x \in \mathbb{R}^d \) be a i.i.d. random vector. Assume that the smaples are i.i.d. from distribution such that \( \mathbb{E}[x_i] = x \) and \( ||x_i|| \leq M\). Then, with probability at least \( 1 - \delta \),
\begin{align*}
    \left\lVert \frac{1}{n}\sum_{i=1}^n x_i - x \right \rVert
    \leq \frac{6M}{\sqrt{n}} \left( 1+ \sqrt{\log (1/\delta)}\right)
\end{align*}
\end{lemma}




\begin{corollary}
 With probability at least \( 1- \delta \),
 \begin{align}
   &  \left\lVert \frac{1}{n}\sum_{i=1}^n x_i - x \right \rVert \nonumber\\
   &\leq  \frac{-L/3 \ln (\delta /(d_1+d_2))+\sqrt{(\ln (\delta /(d_1+d_2))^2 (L/3)^2 - 4\sigma n \ln (\delta /(d_1+d_2)}}{2n} \nonumber
 \end{align}
\end{corollary}
\begin{proof}
 \begin{align*}
      (d_1+d_2) \exp \left(-nt^2/(\sigma + 2Lt/3)\right) = \delta 
 \end{align*}
 Then
 \begin{align*}
  &   -nt^2/(\sigma+2Lt/3) =  \ln (\delta /(d_1+d_2))\\
  & 0 = nt^2 +  2(t L/3) \ln (\delta /(d_1+d_2))  +\sigma \ln (\delta /(d_1+d_2)\\
  & t = \frac{-L/3 \ln (\delta /(d_1+d_2))+\sqrt{(\ln (\delta /(d_1+d_2))^2 (L/3)^2 - 4\sigma n \ln (\delta /(d_1+d_2)}}{2n}
 \end{align*}
\end{proof}
 
 
 \begin{lemma}\label{lem:makrov_iid}
Let \( \mathcal{A}\) be the event such that \( (A_{i_1},A_{i_2},\dots,A_{i_L})\) are independent. Suppose \( \sigma =|| \mathbb{E}[|| A_i^{\top}A_i||]||_2 \) and \( ||A_i||_2 \leq C_A \).
 \end{lemma}
 \begin{proof}
  \begin{align*}
&  \mathbb{E} \left[  \left\lVert A- \frac{1}{L}\sum_{i=1}A_i \right\rVert_2 \right]\\ &= \mathbb{E}\left[\left\lVert A- \frac{1}{L}\sum_{i=1}A_i \right\rVert^2_2\middle | \mathcal{A}\right] \mathbb{P}(\mathcal{A})
  +  \mathbb{E}\left[\left\lVert A- \frac{1}{L}\sum_{i=1}A_i \right\rVert_2 \middle | \mathcal{A}^c \right] \mathbb{P}(\mathcal{A}^c ) \\
  &\leq 
\sqrt{\frac{2\sigma\log(2|\mathcal{S}|)}{n}} + \frac{2C_A\log (2|\mathcal{S}|)}{3n}
  + 2 ||A||_2 (L-1) \mathrm{d}_{\mathrm{mix}} \left( \frac{N}{L} \right)
 \end{align*}
 \end{proof}
 
 \begin{lemma}
 Let \( X_0,\dots, X_N \) be stationary finite Markov chain. Randomly sample \( X_{i_1},\dots,X_{i_L}\). Let \((\tilde{X}_{i_1},\dots,\tilde{X}_{i_L}) \) be a i.i.d. sequence sampled from stationary distribution. Then,
 \begin{align*}
     \mathbb{P}\left( (X_{i_1},\dots,X_{i_L}) \neq (\tilde{X}_{i_1},\dots,\tilde{X}_{i_L}) \right) \leq \sum_{i=1}^{N-1} d_{\mathrm{TV}}(d_i)
 \end{align*}
 \end{lemma}
 \begin{proof}
 \begin{align} 
    \sum_{M_k} \mathbb{P}\left( (X_{i_1},\dots,X_{i_L}) \neq (\tilde{X}_{i_1},\dots,\tilde{X}_{i_K}) \right\mid M_k)\mathbb{P}(M_k) &\leq \sum_{M_k}\sum_{i=1}^{L-1} d_{\mathrm{TV}}(d_{k_i}) \mathbb{P}(M_k) \nonumber\\
    &= \sum_{M_k}\sum_{i=1}^{L-1} c \rho^{d_{k_i}} \mathbb{P}(M_k) \nonumber\\
    &= \sum_{d=1}^{N-1} c\rho^d \frac{\sum_{k,i}1(d_{k_i}=d)}{\binom{N}{L}} \nonumber\\
    &= \sum_{d=1}^{N-1} c\rho^d \frac{2(N-d)}{\binom{N}{2}} \nonumber
 \end{align}
 where \( d_j = |i_{j+1}-i_j| \).
 \end{proof}
 
 
 \begin{lemma}
 Let \( (X_{i_1},X_{i_2},\dots,X_{i_k}) \) be Markov chain sampled from stationary distribution. Then
 \end{lemma}
 \begin{proof}
 \end{proof}
 
 \begin{lemma}[Time difference between samples]
 \end{lemma}
 \begin{proof}
The number of unique indices is
 \begin{align}
    \sum_{\sigma} 1(d_{\sigma_i}=1) = 
 \end{align}
 \end{proof}
 
\section{Stacking vectors}
Let 
\begin{align*}
    X_{k+1}  =     \begin{bmatrix}
    V_{k+1}\\
    V_{k-1}\\
    \vdots\\
    V_{k-N+2}
    \end{bmatrix}
    \in \mathbb{R}^{|S|N} \nonumber
\end{align*}

\begin{align}
X_{k+1}
    &= X_k 
    +  \nonumber
\end{align}






\begin{lemma}
    Proof on second moment using high probability bound
\end{lemma}

\begin{proof}
    Let 
\begin{align*}
    \mathcal{A}:= 
    \left\{ 
    \left\lVert
\frac{1}{L}\sum^L_{i=1}
  (e^k_{s_i}e^{k\top}_{s_i}-\tilde{D}_k)\right\rVert_2 \leq 
  \frac{6}{\sqrt{L}} \left( 1+ \sqrt{\log (1/\delta_1)}\right)
    \right\}.
\end{align*}

Using~\Cref{lem:concentration_iid}, we can see that
\begin{align}
  &\mathbb{E}
\left[ \left\lVert
\frac{1}{L}\sum^L_{i=1}
  (e^k_{s_i}e^{k\top}_{s_i}-\tilde{D}_k)\right\rVert^2_2
\right] \nonumber \\
&\leq \mathbb{E}
\left[ \left\lVert
\frac{1}{L}\sum^L_{i=1}
  (e^k_{s_i}e^{k\top}_{s_i}-\tilde{D}_k)\right\rVert^2_2
\middle | A\right ]\mathbb{P}(A)
+ 
\mathbb{E}
\left[ \left\lVert
\frac{1}{L}\sum^L_{i=1}
  (e^k_{s_i}e^{k\top}_{s_i}-\tilde{D}_k)\right\rVert^2_2
\middle | A^c \right] \mathbb{P}(A^c) \nonumber \\
&\leq 
 \frac{-1/3 \ln (\delta /|\mathcal{S}|)+\sqrt{(\ln (\delta /|\mathcal{S}|))^2 (1/3)^2 - 4\sigma L \ln (\delta /|\mathcal{S}|)}}{2L}
+ 2\delta_1 \nonumber
\end{align}

The last inequality follows from Cauchy-Schwartz inequality:
\begin{align*}
    \left\lVert
\frac{1}{L}\sum^L_{i=1}
  (e^k_{s_i}e^{k\top}_{s_i}-\tilde{D}_k)\right\rVert^2_2 \leq \frac{1}{L^2}\left(L \sum^L_{i=1}   ||e^k_{s_i}e^{k\top}_{s_i}-\tilde{D}_k||^2_2 \right) \leq 4.
\end{align*}
Now we bound \( \mathbb{E}\left[\left\lVert
     \Delta_{\infty}(V_k) - \Delta_k (V_k)
     \right\rVert^2_2
     \middle|
     \mathcal{F}_{k-1}
     \right] \).
\begin{align*}
    &\mathbb{E}\left[ 
    || (D_{\infty}- \tilde{D}_k)V_k
    +\gamma (D_{\infty}P - \tilde{D}_kP_k)V_k
    +
    (D_{\infty}-\tilde{D}_k)R||^2_2 
    \mid \mathcal{F}_{k-1}\right]\\
    &
    \leq 
    2||V||_2^2\mathbb{E}
    \left(\left[ 
    ||D_{\infty}-\tilde{D}_k||^2_2
    + 
    ||D_{\infty}P-D_{k}P_k||^2 \mid \mathcal{F}_{k-1}
    \right]
    \right)\\
 &\mathbb{E}\left[ 
    || (D_{\infty}- \tilde{D}_k)V_k
    +\gamma (D_{\infty}P - \tilde{D}_kP_k)V_k
    +
    (D_{\infty}-\tilde{D}_k)R||^2_2 
    \right]   \\
    &\leq 2 (\mathbb{E}\left[\left\lVert (D_{\infty}- \tilde{D}_k)V_k
    +\gamma (D_{\infty}P - \tilde{D}_kP_k\right)V_k \right\rVert^2]
    + \mathbb{E}[\left\lVert (D_{\infty}-\tilde{D}_k)R \right\rVert^2]\\
    &\leq 
    2(||V||^2_2+R_{\max}) 
    \left ( 
    ||D_{\infty}-\tilde{D}_k||^2_2\right)
    + 
    2\gamma ||V||^2_2 \left \lVert D_{\infty}P - \tilde{D}_kP_k \right \rVert^2_2
\end{align*}


How do we bound \( \mathbb{E}\left[\left\lVert D_{\infty} - \tilde{D}_k \right\rVert^2_2\right] \) ?

\begin{align*}
&    \mathbb{E}\left[ \left\lVert D_{\infty} - \frac{1}{N}\sum_{i=1}^N e_i^{\top}e_i \right\rVert^2_2\right] \\
&\leq 2 \left( \mathbb{E}\left[ \left\lVert D_{\infty} - D_k \right\rVert^2_2 \right]
+\mathbb{E}\left[ \left\lVert  D_k - \frac{1}{N}\sum_{i=1}^N e_i^{\top}e_i \right\rVert^2_2 \right]
\right)
\\
& \leq 2\left( ||D_{\infty}-D_k||^2_2 + N \sum_i \mathbb{E}\left[ \left\lVert \frac{1}{N} D_k -\frac{1}{N}e_ie_i^{\top}\right\rVert^2 \right]\right)
\end{align*}

\end{proof}



\begin{algorithm}[H]
\caption{TD experience replay buffer}
\begin{algorithmic} 
\REQUIRE $B_{-1}:=X_{-N},X_{-N+1},\dots,X_{-1}$ data samples $V_0$;
\STATE $k=0$;
\FOR{$k\leq T$}
    \STATE Sample $O_k \sim \mu_{\infty} $
    \STATE $B_k  \leftarrow B_{k-1}\setminus \{ O_{k-N} \} \cup \{O_k\}$
    \STATE Sample $M_k\sim B_k$
     \STATE Set $V^{M_k}_0 = V_k$
    \FOR{$i \leq L$}
    \STATE Update $V^{M_k}_{i+1}\leftarrow V_i^{M_k}+\alpha_k (A(V_k^{M_k}-V^{\pi})+w(O^{M_k}_i,V^{M_k})$ 
    \STATE $i\leftarrow i+1$
    \ENDFOR
    \STATE Set $V_{k+1}=V^{M_k}_{L-1}$
\ENDFOR
\end{algorithmic}
\end{algorithm}


\section{i.i.d. case}
\import{./}{iid}
\section{Coupling}
\import{./}{coupling}
\section{Markovian case}
\import{./}{markovian}

\section{i.i.d. sampling without replacement}
\import{iid}{wo_replacemnt}

\section{Batch}
\import{./}{batch}




